Leader: Prefixing a Length for Faster Word Vector Serialization

Two competing file formats have become the de facto standards for distributing pre-trained word embeddings. Both are named after the most popular pre-trained embeddings that are distributed in that format. The GloVe format is an entirely text based format that suffers from huge file sizes and slow reads, and the word2vec format is a smaller binary format that mixes a textual representation of words with a binary representation of the vectors themselves. Both formats have problems that we solve with a new format we call the Leader format. We include a word length prefix for faster reads while maintaining the smaller file size a binary format offers. We also created a minimalist library to facilitate the reading and writing of various word vector formats, as well as tools for converting pre-trained embeddings to our new Leader format.

==> outline.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{ll|rr|rr}
                       &        & \multicolumn{2}{c|}{Gensim} & \multicolumn{2}{c}{Ours} \\
        Pre-trained    & Format & Mean         & Std         & Mean        & Std        \\
        \hhline{==|====}
        GloVe-6B       & Text   & 37.58        & 1.03        &  11.15      & 0.10       \\
                       & W2V    & 2.50         & 0.08        &   1.97      & 0.12       \\
        \hline
        GloVe-27B      & Text   & 210.47       & 6.70        &  62.06      & 1.05       \\
                       & W2V    & 7.52         & 0.31        &   6.97      & 0.09       \\
        \hline
        GloVe-42B      & Text   & 484.95       & 1.77        &  138.53     & 2.30       \\
                       & W2V    & 12.93        & 0.17        &   11.22     & 0.28       \\
        \hline
        GloVe-840B     & Text   & 554.43       & 5.61        &  154.12     & 0.33       \\    
                       & W2V    & 14.90        & 0.12        &   12.92     & 0.35       \\
        \hline
        FastText Wiki  & Text   & 243.63       & 4.11        &  66.97      & 0.08       \\
                       & W2V    & 6.85         & 0.22        &   5.82      & 0.19       \\
        \hline
        FastText Crawl & Text   & 484.71       & 5.40        &  136.86     & 2.14       \\
                       & W2V    & 13.57        & 0.35        &   11.53     & 0.15       \\
        \hline
        Google News    & Text   & 782.46       & 61.85       &  357.26     & 7.16       \\   
                       & W2V    & 21.54        & 0.81        &   19.41     & 0.25       \\
    \end{tabular}
    \caption{
        Given that our numbers are in the table above maybe we can show gensim mean + std and a $\Delta$ to us?
    }
    \label{tab:gensim-bakeoff-repeat}
\end{table}

\begin{itemize}
    \item Readings for all the formats
    \item Writing for all formats
    \item Conversion between formats
    \item Sniffing a file to determining the format
    \item Benchmark reading against Gensim? This would go in the discussion of the library rather
        than the benchmark section because that is about comparing file formats while this is just
        a good point of our library.
    \item Look at using \texttt{fadvise} and \texttt{madvise} to speed things up
    \item Use github actions to test on Mac and Windows too.
    \item Host Leader versions of of common vectors somewhere? A new dropbox? Github? S3?
    \item Add tests on the dispatching functions
    \item Tests for user vocabs?
    \item Add FastText and FastTextBin to the Enum? Some sort of aliasing? In sniffing we should
        just return word2vec instead of trying to pick one. On the dispatch we should dispatch
        these too the same way.
    \item Look into renaming the Dense vectors
\end{itemize}

\begin{itemize}
    \item Conclusion
    \begin{itemize}
        \item Outlined short-comings in common word vector formats
        \item Introduced our format that fixes most of these problems
        \item Provide a library for read, writing, and converting between these formats
        \begin{itemize}
            \item Regardless of adoption of the new format we have provided an easy to use, small library for working with binary word2vec files and we should at least move to those over glove files)
        \end{itemize}
        \item Provided benchmarks about reading
    \end{itemize}
    \item Future Work
    \begin{itemize}
        \item File-backed on-the-fly vector reading vectors from file.
    \end{itemize}
\end{itemize}

\begin{itemize}
    \item Table and graphs that compare the same vocab and vectors data in each format
    \begin{itemize}
        \item GloVe
        \item Word2Vec Binary
        \item Word2Vec Text
        \item Leader
    \end{itemize}
    \item File Size vs:
    \begin{itemize}
        \item vocab size
        \item max length of the word
        \item Vector size should have the same growth across all formats. I want to confirm this and then
            have a small mention in the caption of the table
        \item Include a table for common pre-trained embeddings
    \end{itemize}
    \item Read Time vs:
    \begin{itemize}
        \item vocab size
        \item vector size
        \item max length of the word
        \item Include a table for common pre-trained embeddings
    \end{itemize}
    \item Given common real pre-trained embeddings how many padding characters are there vs the actual
        token characters
    \item Include system stats
    \begin{itemize}
        \item Intel(R) Core(TM) i7-7700HQ CPU @ 2.80GHz
        \item 8 cores
        \item 6144 KB cache
        \item 32819844 kB RAM
        \item python 3.6.10 as installed by anaconda
        \item word-vectors 4.0.0 (installed from PyPi)
        \item numpy 1.18.5 (installed by anaconda)
        \item gensim 3.8.3 (installed from anaconda)
    \end{itemize}
    \item Clearing the system cache \texttt{sync; echo 2 > /proc/sys/vm/drop\_caches} to clear PageCache, dentries and inodes.
\end{itemize}

\begin{itemize}
    \item Header $\rightarrow$ \texttt{Magic Number, Vocab Size, Vector Size, Max Length}
    \item Little endian encoded longs longs
    \item Binary word padded out to \texttt{Max Length} followed by binary vector (specified endianess?)
    \item Draw Backs:
    \begin{itemize}
        \item Possible drawback: you can't look at that head of the file manually (in vim) to see the size?
        \begin{itemize}
            \item Glove $\leftarrow$ \texttt{wc -l file}
            \item w2v $\leftarrow$ \texttt{head -n 1 file}
            \item Dense $\leftarrow$ \texttt{od -l --endian=little -N 32 file}
            \end{itemize}
        \item It is a little larger than the word2vec format
        \item Can be slower when the number of padded bytes is massive. (The time for the strip makes it slower
              than the iteration through? Look at prefixing the line with the word length to speed it up?) prefixing
              line with the length made it a lot faster, is faster than w2v on most datasets and comparable on the
              last two. The probably datasets are both common crawl datasets from glove which has massive tokens of
              random shit in them.
    \end{itemize}
\end{itemize}

\begin{itemize}
    \item GloVe
    \begin{itemize}
        \item Fat files
        \item slow load
        \item Word2Vec Text is the same but for the first line
    \end{itemize}
    \item Word2Vec
    \begin{itemize}
        \item Iterating thought the word to find the space is slow
        \item Binary format is scary to most people
    \end{itemize}
    \item Senna \cite{JMLR:v12:collobert11a}
    \begin{itemize}
        \item You are still fat because of the text based
        \item You need to keep track of 2 files
    \end{itemize}
    \item Libraries
    \begin{itemize}
        \item Hidden deep in large libraries with a lot of baggage
        \item Returns library specific objects that are more complex than they really need to be
        \item Gensim \cite{rehurek_lrec}
        \item Baseline \cite{presselBaselineLibraryRapid2018}
    \end{itemize}
    \item Bugs
    \begin{itemize}
        \item Simplicity of the text formats leads to people not thoroughly testing
        \item You can have characters other than \texttt{" "} in the word that causes a split in
            the token when you just call \texttt{.split()}
        \item Find stats on how many pre-trained embeddings have these symbols
        \item Some pre-trained embeddings have duplicated tokens. This causes a gap in the word
            to index mapping and there are extra vectors in the output
        \item See how many of these there are.
    \end{itemize}
    \item Vectors are often described by the format of the most common pre-trained embeddings that use
        that format. They don't describe the format at all
    \begin{itemize}
        \item The real data structure of the embeddings in memory is associated arrays which is how
            it is on disk
        \item Some have the meta data removed?
        \item Is the removal of meta data because of the of the rise of dynamic languages? The
            ease of \texttt{list.append()} in python?
        \item FastText uses the word2vec text format so these names don't really work
    \end{itemize}
    \item Look up the Vowpal Rabbit format
\end{itemize}

\begin{itemize}
    \item What are word vectors from an NLP sense?
    \item What is the real word vector data structure? A dict? associated arrays?
    \item What are the common file formats? and who uses them?
    \begin{itemize}
        \item GloVe \cite{penningtonGloVeGlobalVectors2014}
        \begin{itemize}
            \item GloVe
        \end{itemize}
        \item word2vec binary
        \begin{itemize}
            \item Word2Vec \cite{mikolovEfficientEstimationWord2013, mikolovDistributedRepresentationsWords2013}
            \item Need to lookup how well specified this format is, it seems just encoded in the
                software talk about how this makes other implementations harder and scarier. They don't specify it
                in the paper and the code doesn't seem to specify endinness 
            \item How is the header encoded? Binary numbers or as text? <- as text
        \end{itemize}
        \item word2vec text
        \begin{itemize}
            \item FastText use \cite{bojanowskiEnrichingWordVectors2017} for the description of the vectors
                  and \cite{mikolovAdvancesPreTrainingDistributed2018} for the pre-trained ones
            \item numberbatch \cite{speer2017conceptnet}
        \end{itemize}
        \item Senna \cite{JMLR:v12:collobert11a}
        \begin{itemize}
            \item Two file text
            \item One is the vector file which is text based
            \item the Other is the word file which is text based
            \item aligned by their lines
        \end{itemize}
    \end{itemize}
\end{itemize}
